Robust Body Exposure (RoBE): A Graph-based Dynamics Modeling Approach to Manipulating Blankets over People

Robotic caregivers could potentially improve the quality of life of many who require physical assistance. However, in order to assist individuals who are lying in bed, robots must be capable of dealing with a significant obstacle: the blanket or sheet that will almost always cover the person's body. We propose a method for targeted bedding manipulation over people lying supine in bed where we first learn a model of the cloth's dynamics. Then, we optimize over this model to uncover a given target limb using information about human body shape and pose that only needs to be provided at run-time. We show how this approach enables greater robustness to variation relative to geometric and reinforcement learning baselines via a number of generalization evaluations in simulation and in the real world. We further evaluate our approach in a human study with 12 participants where we demonstrate that a mobile manipulator can adapt to real variation in human body shape, size, pose, and blanket configuration to uncover target body parts without exposing the rest of the body. Source code and supplementary materials are available online.

==> coverletter.tex <==
% Version Submitted for Initial Submission
% Dear Dr. Asfour,

% I am enclosing a manuscript entitled "Robust Body Exposure (RoBE): A Graph-based Dynamics Modeling Approach to Manipulating Blankets over People" for consideration for publication as a journal article in IEEE Robotics and Automation Letters. In our paper, we present a new, graph-based technique for robotic bedding manipulation over people in which a robot uncovers a blanket from a target body part while ensuring the rest of the human body remains covered.

% With this submission, I, as corresponding author on behalf of all the authors, confirm that this manuscript represents original research of which all authors played a significant role. This manuscript has not been published elsewhere, accepted for publication elsewhere, or under editorial review for publication elsewhere.

% Thank you for your time and consideration.

% Warm regards,
% Kavya Puthuveetil


% Version Submitted for Resubmission
% Dear Dr. Asfour,

% I am enclosing the revised version of a manuscript entitled "Robust Body Exposure (RoBE): A Graph-based Dynamics Modeling Approach to Manipulating Blankets over People" for consideration for publication as a journal article in IEEE Robotics and Automation Letters. In our paper, we present a new, graph-based technique for robotic bedding manipulation over people in which a robot uncovers a blanket from a target body part while ensuring the rest of the human body remains covered.

% In this revised version of the letter, we have made a number of changes to incorporate the reviewers' comments. In particular, we have expanded our discussion of the SOTA and clarified how we transfer simulation-trained dynamics models to the real world. We also generally clarified the text and figures as requested by the reviewers.

% With this submission, I, as corresponding author on behalf of all the authors, confirm that this manuscript represents original research of which all authors played a significant role. This manuscript has not been published elsewhere, accepted for publication elsewhere, or under editorial review for publication elsewhere.

% Thank you for your time and consideration.

% Warm regards,
% Kavya Puthuveetil


Version Submitted for Final
Dear Dr. Asfour,

I am enclosing the final version of a manuscript entitled "Robust Body Exposure (RoBE): A Graph-based Dynamics Modeling Approach to Manipulating Blankets over People" for consideration for publication as a journal article in IEEE Robotics and Automation Letters. In our paper, we present a new, graph-based technique for robotic bedding manipulation over people in which a robot uncovers a blanket from a target body part while ensuring the rest of the human body remains covered.

In this final version of the letter, we have adjusted our contributions, as suggested by the reviewers, to better highlight the technical novelty of our work and the improvements of our method on other existing approaches.

With this submission, I, as corresponding author on behalf of all the authors, confirm that this manuscript represents original research of which all authors played a significant role. This manuscript has not been published elsewhere, accepted for publication elsewhere, or under editorial review for publication elsewhere.

Thank you for your time and consideration.

Warm regards,
Kavya Puthuveetil


